Factorization-based Lossless Compression of Inverted Indices

Many large-scale Web applications that require ranked top-k retrieval such as Web search and online advertising are implemented using inverted indices. An inverted index represents a sparse term-document matrix, where non-zero elements indicate the strength of term-document association. In this work, we present an approach for lossless compression of inverted indices. Our approach maps terms in a document corpus to a new term space in order to reduce the number of non-zero elements in the term-document matrix, resulting in a more compact inverted index. We formulate the problem of selecting a new term space that minimizes the resulting index size as a matrix factorization problem, and prove that finding the optimal factorization is an NP-hard problem. We develop a greedy algorithm for finding an approximate solution. A side effect of our approach is increasing the number of terms in the index, which may negatively affect query evaluation performance. To eliminate such effect, we develop a methodology for modifying query evaluation algorithms by exploiting specific properties of our compression approach. Our experimental evaluation demonstrates that our approach achieves an index size reduction of 20%, while maintaining the same query response times. Higher compression ratios up to 35% are achievable, however at the cost of slightly longer query response times. Furthermore, combining our approach with other lossless compression techniques, namely variable-byte encoding, leads to index size reduction of up to 50%.

==> related_works.tex <==

\section{Related Work}
\label{sec:relwork}
% Bi-clustering with coherent values
% NMF, SVD
% lossless compression techniques

%In this section, we contrast our approach with other related work. % in the areas of lossless compression, matrix factorization, biclustering and lossy compression.

% \subsection{Lossless Compression Techniques}

Lossless compression of inverted indices has been an active topic for the past few years. Most of the developed techniques (e.g., variable-byte encoding, gamma-coding and delta-coding \cite{delta,Scholer02}) aim at generating an efficient encoding of the entries in posting list, and thus can be integrated with our approach (cf. Section~\ref{sec:expr}). % that variable-byte encoding can achieve a reasonable compression efficiency, even when compressing indices resulting from our algorithm. We anticipate that other lossless compression algorithms would exhibit the same behavior when integrated with our approach.

There are multiple techniques for lossy compression. One of the widely used techniques is \emph{static pruning} \cite{sp2,sp1}. Techniques that are based on static pruning truncate postings that have low impact on the results of top-$k$ queries. The simplest form is to remove postings with payload values less than a specific cut-off threshold. Clearly, lossy compression might lead to degradation in results quality, unlike lossless compression where quality of results is not affected. In general, lossy compression can be integrated with lossless compression techniques in order to achieve higher compression ratios at the cost of lowering the quality of query results.

%\subsection{Matrix Factorization Techniques}

Several matrix factorization approaches have been proposed such as Non-negative Matrix Factorization \cite{nmf2,nmf1,LYF10}, Principal Component Analysis \cite{PCA}, K-means clustering \cite{Kmeans}, Latent Semantic Analysis \cite{LSA}, and Singular Value Decomposition \cite{SVD}. The goal of these techniques is to factor a given matrix into two (or three) factor matrices that (optionally) exhibit some level of sparseness.  Such techniques  provide a \emph{close approximation} of the input matrix, while our approach provides an \emph{exact} factorization of the input matrix. %That is, NMF algorithms (and other variants) minimize the distance between the input matrix and the product of the resulting matrices (for some distance function), but there is no guarantee that the distance is be zero (i.e., lossless).
Modifying NMF algorithms to be lossless is not straightforward. For example, one na\"{\i}ve approach is to compute the remainder matrix $R = V-WH$ so that the matrix $V$ can be compactly represented using the matrices $W,$ $H$, and $R$ (i.e., $V = WH +R$). Unfortunately, there is no guarantee that sparseness of $W$ and $H$ would lead to sparseness of $R$. In fact, the size of $R$ can be larger than the size of $V$ because elements in $V$ with values equal to zero may have non-zero values in the product $WH$. % which in turn requires adding extra negative elements to the matrix $R$.

% Furthermore, current matrix factorization approaches impose a constraint on the rank of the obtained factors, which is typically smaller than the rank of the input matrix. Clearly, such constraint is unnecessary for the application of inverted index compression and might lead to suboptimal compression ratios.

%\bigskip

Another line of related work in a different context, namely signal and image processing,
considers a problem of representing a {\em signal} (vector) using a linear
combination of a small number of basis vectors from a {\em dictionary} (e.g., \cite{Aharon06,Tropp04}).
The problem of selecting the optimal dictionary given the set of signals is
similar to the problem we consider, with two major differences:
(1) the dimensions of the factor matrices are selected in advance, and
(2) the sparseness is required only from the encoding vectors (matrix $W$) and not from the basis vectors (matrix $H$).
%It is shown that even encoding a single input signal optimally given a dictionary is NP-hard~\cite{DMA97},
%unless the dictionary has certain properties.

% Greedy approximation algorithms for the problem of dictionary selection, such as K-SVD~\cite{AEB05},
% start with some lossy approximation of $V$ by $W_0 H_0$ and iteratively improve the solution by
% adding and modifying basis vectors so as to minimize the residual. This is inefficient in our setting due to the same factor
% that deems standard \emph{approximate} factorization techniques inefficient -- prohibitive
% cost of working with the (not necessarily sparse) residual. An essential feature of the algorithm we propose is that it maintains lossless {\em and} sparse representation throughout the computation.


%\subsection{Biclustering Techniques}


Another related problem is discovering biclusters in two-dimensional data (refer to \cite{BICLUSTER} for a comprehensive survey). % A bicluster in a matrix is identified by a set of rows and a set of columns.
The goal is to discover the largest bicluster (submatrix) that exhibits certain characteristics (e.g., have the same value, or follow additive/multiplicative patterns). Computing the largest bicluster is shown to be NP-hard \cite{BICLUSTER}. Our approach can be viewed as a biclustering problem (however, with a different goal) as follows.  Each meta-term $\tau$ represents a bicluster in $V$ whose rows are multiples of each other and contain non-zero values only. Each bicluster results in a number of non-zero elements in matrix $W$ (respectively, $H$) that is equal to the number of rows (respectively, columns) of the bicluster. The size of a bicluster is defined as the total number of the contained rows and columns. Our goal is to obtain a set of disjoint biclusters that covers all non-zero elements of the input matrix such that the total size of biclusters is minimal. Unfortunately, previous approaches for discovering biclusters cannot be easily extended to address the described objective function.

% \subsection{Lossy Compression Techniques}
%



% TODO: add a note similar to : "More recently, Buttcher and Clarke considered index pruning specifically so that the resulting index would fit in memory, although supplemental disk indices are sometimes used for additional information. Query performance improves in part because of memory speed and in part because the smaller amount of data, although these different factors were not analyzed in detail" 
